Integrated Study of NGC 1662, NGC 1778, NGC 2422, and NGC 2437 Open Clusters: from Stellar Parameters to Orbital Trajectories Utilizing Gaia DR3 Archive

We present a comprehensive photometric, astrometric, and dynamical study of four Galactic open clusters, NGC 1662, NGC 1778, NGC 2422, and NGC 2437, using Gaia DR3 data. Probable cluster members were identified through astrometric and photometric criteria. Radial density profiles were modelled with a King-type surface-density distribution to derive structural parameters. Mean parallaxes and proper motions yielded astrometric distances of 410 +/- 12 pc (NGC 1662), 1761 +/- 335 pc (NGC 1778), 477 +/- 18 pc (NGC 2422), and 1681 +/- 172 pc (NGC 2437). Fundamental astrophysical parameters were estimated through Bayesian isochrone fitting using PARSEC evolutionary models within an MCMC framework. The resulting ages (log(t/yr)) are 8.91 (-0.33/+0.24), 8.20 (-0.11/+0.18), 7.80 (-0.11/+0.06), and 8.56 (-0.34/+0.27), respectively. Luminosity functions were transformed into present-day mass functions using an isochrone-based mass-luminosity relation. The derived mass-function slopes are broadly consistent, within uncertainties, with the classical Salpeter form. Mean systemic radial velocities from Gaia DR3 and complementary spectroscopic surveys enabled the determination of Galactic space velocities (U, V, W) in the Local Standard of Rest frame. Backward orbital integrations over 3 Gyr were performed using galpy with the MWPotential2014 Galactic potential. The resulting orbits are nearly circular (e <= 0.106), with limited vertical excursions (Z_max < 0.3 kpc), consistent with thin-disc kinematics. Inferred birth radii suggest possible outward radial displacement for NGC 2422, NGC 2437, and NGC 1778, and inward displacement for NGC 1662. Overall, all four clusters appear to have evolved within relatively stable Galactic disc orbits.

==> Supplementary_File_Electronic_Table.tex <==
\begin{table*} \footnotesize
\centering
\caption{Radial velocity measurements for NGC 1662}
\begin{tabular}{l c c c c c c c c l}
%\begin{tabularx}{\linewidth}{l c c c c c c c c l}
\hline\hline
ID & $\alpha$ (hh:mm:ss) & $\delta$ (dd:mm:ss) & $G$ (mag) & $P$ & $V_R$ (km s$^{-1}$)& $\sigma_{V_R}$ & & RUWE & Survey \\
\hline
1 & 04:46:38.00 & +10:39:53.9 & 14.81 & 0.96 & -1.07 & 6.78 & & 1.02 & Gaia DR3 \\
2 & 04:46:42.44 & +11:08:50.5 & 11.81 & 1.00 & -12.67 & 1.90 & & 1.14 & LAMOST \\
3 & 04:46:47.24 & +10:37:55.2 & 12.71 & 1.00 & -13.11 & 2.08 & & 1.00 & LAMOST \\
4 & 04:46:50.04 & +11:10:47.6 & 13.74 & 0.97 & -19.47 & 4.41 & & 1.14 & Gaia DR3 \\
5 & 04:46:51.19 & +11:19:54.0 & 11.64 & 1.00 & -7.68 & 5.29 & & 1.19 & LAMOST \\
6 & 04:47:04.93 & +11:22:59.0 & 14.56 & 1.00 & -7.18 & 4.96 & & 0.98 & LAMOST \\
7 & 04:47:16.87 & +10:43:26.1 & 10.12 & 0.98 & -21.73 & 3.22 & & 1.16 & Gaia DR3 \\
8 & 04:47:29.10 & +10:50:44.9 & 14.30 & 1.00 & -9.85 & 4.01 & & 1.38 & LAMOST \\
9 & 04:47:30.71 & +11:44:18.5 & 13.23 & 1.00 & -11.47 & 2.18 & & 1.07 & LAMOST \\
10 & 04:47:43.17 & +10:40:51.8 & 14.69 & 0.98 & -21.34 & 8.11 & & 0.97 & Gaia DR3 \\
11 & 04:47:43.56 & +10:39:05.2 & 14.08 & 1.00 & -15.56 & 2.98 & & 1.01 & LAMOST \\
12 & 04:47:46.85 & +10:20:03.3 & 9.35 & 0.95 & -17.75 & 1.86 & & 0.94 & Gaia DR3 \\
13 & 04:47:47.13 & +10:52:39.6 & 13.94 & 0.98 & -12.18 & 2.75 & & 1.02 & Gaia DR3 \\
14 & 04:47:48.31 & +10:38:32.7 & 13.72 & 0.98 & -13.92 & 2.55 & & 1.00 & Gaia DR3 \\
15 & 04:47:49.62 & +11:04:25.3 & 13.95 & 1.00 & -10.27 & 2.76 & & 1.15 & LAMOST \\
16 & 04:47:52.01 & +10:47:05.2 & 13.96 & 1.00 & -10.46 & 3.88 & & 1.04 & LAMOST \\
17 & 04:47:53.04 & +10:52:58.4 & 11.35 & 1.00 & -21.72 & 4.67 & & 1.14 & Gaia DR3 \\
18 & 04:47:53.33 & +10:52:34.3 & 15.08 & 1.00 & -16.94 & 5.24 & & 1.04 & LAMOST \\
19 & 04:47:55.68 & +11:52:53.0 & 13.28 & 1.00 & -12.59 & 2.34 & & 1.06 & LAMOST \\
20 & 04:48:00.57 & +10:57:10.7 & 10.06 & 0.99 & -13.55 & 1.14 & & 0.99 & Gaia DR3 \\
21 & 04:48:04.94 & +10:59:21.2 & 11.59 & 1.00 & -13.13 & 0.83 & & 1.01 & Gaia DR3 \\
22 & 04:48:09.46 & +10:51:52.0 & 14.54 & 0.99 & -11.98 & 4.40 & & 1.03 & Gaia DR3 \\
23 & 04:48:09.87 & +11:35:44.2 & 14.31 & 1.00 & -14.39 & 3.07 & & 1.10 & LAMOST \\
24 & 04:48:10.86 & +11:40:12.5 & 11.63 & 1.00 & -11.85 & 3.08 & & 1.10 & LAMOST \\
25 & 04:48:15.12 & +11:00:33.8 & 11.22 & 0.99 & -15.78 & 1.37 & & 1.13 & Gaia DR3 \\
26 & 04:48:25.18 & +10:47:05.8 & 10.67 & 0.99 & -19.08 & 1.60 & & 1.02 & Gaia DR3 \\
27 & 04:48:25.49 & +10:36:36.8 & 14.26 & 0.98 & -13.40 & 4.30 & & 1.11 & Gaia DR3 \\
28 & 04:48:27.36 & +10:49:48.3 & 10.98 & 1.00 & -13.27 & 1.65 & & 1.05 & LAMOST \\
29 & 04:48:27.51 & +11:13:33.9 & 13.78 & 1.00 & 8.59 & 3.67 & & 1.02 & LAMOST \\
30 & 04:48:27.87 & +10:55:45.7 & 10.24 & 0.98 & -25.95 & 3.40 & & 1.02 & Gaia DR3 \\
31 & 04:48:29.51 & +10:55:48.3 & 7.95 & 1.00 & -13.76 & 0.12 & & 0.95 & Gaia DR3 \\
32 & 04:48:32.08 & +10:57:59.0 & 8.42 & 1.00 & -12.90 & 0.12 & & 0.94 & Gaia DR3 \\
33 & 04:48:32.13 & +11:35:51.9 & 11.87 & 1.00 & -12.61 & 3.33 & & 1.19 & Gaia DR3 \\
34 & 04:48:33.82 & +10:55:52.8 & 14.51 & 0.97 & -13.11 & 3.66 & & 1.04 & Gaia DR3 \\
35 & 04:48:35.45 & +11:00:17.0 & 13.36 & 0.99 & -13.18 & 1.83 & & 1.03 & Gaia DR3 \\
36 & 04:48:37.75 & +11:23:23.2 & 14.83 & 0.97 & -8.67 & 4.51 & & 1.09 & Gaia DR3 \\
37 & 04:48:41.96 & +10:53:54.1 & 13.09 & 1.00 & -9.72 & 1.65 & & 1.01 & LAMOST \\
38 & 04:48:42.21 & +10:59:33.3 & 10.60 & 0.99 & -19.14 & 2.62 & & 0.93 & Gaia DR3 \\
39 & 04:48:42.94 & +10:25:20.4 & 14.90 & 0.98 & -20.75 & 5.40 & & 1.01 & Gaia DR3 \\
40 & 04:48:43.30 & +10:50:32.0 & 12.07 & 1.00 & -9.73 & 1.40 & & 1.06 & LAMOST \\
41 & 04:48:43.43 & +11:33:04.0 & 12.38 & 1.00 & -9.48 & 2.42 & & 0.95 & Gaia DR3 \\
42 & 04:48:49.01 & +10:29:36.7 & 14.74 & 0.98 & -15.41 & 7.02 & & 0.99 & Gaia DR3 \\
43 & 04:48:50.04 & +10:57:34.1 & 14.05 & 1.00 & -12.29 & 2.47 & & 1.06 & LAMOST \\
44 & 04:48:51.15 & +10:32:08.8 & 15.33 & 0.97 & -3.71 & 5.86 & & 1.10 & Gaia DR3 \\
45 & 04:48:53.68 & +10:42:42.2 & 11.65 & 1.00 & -12.79 & 0.50 & & 1.28 & LAMOST \\
46 & 04:48:55.92 & +11:12:50.9 & 12.79 & 1.00 & -12.26 & 2.60 & & 1.00 & Gaia DR3 \\
47 & 04:48:58.17 & +10:54:33.3 & 13.76 & 1.00 & -11.94 & 1.95 & & 0.99 & LAMOST \\
48 & 04:48:59.71 & +11:48:17.2 & 13.39 & 1.00 & -12.91 & 2.73 & & 0.98 & LAMOST \\
49 & 04:49:01.21 & +11:41:57.2 & 14.70 & 0.95 & -13.31 & 4.48 & & 1.08 & Gaia DR3 \\
50 & 04:49:02.62 & +10:14:32.4 & 12.18 & 1.00 & -3.93 & 4.00 & & 0.98 & Gaia DR3 \\
51 & 04:49:03.20 & +11:01:51.0 & 13.96 & 1.00 & -11.42 & 2.54 & & 1.01 & LAMOST \\
52 & 04:49:04.61 & +11:40:09.7 & 11.10 & 0.97 & -20.73 & 3.47 & & 1.17 & Gaia DR3 \\
53 & 04:49:06.82 & +10:40:27.9 & 13.73 & 1.00 & -14.59 & 2.99 & & 1.39 & LAMOST \\
54 & 04:49:07.18 & +10:42:48.1 & 12.37 & 1.00 & -13.75 & 3.44 & & 1.30 & Gaia DR3 \\
55 & 04:49:07.69 & +10:15:53.6 & 14.70 & 0.92 & -3.03 & 9.10 & & 0.99 & Gaia DR3 \\
56 & 04:49:10.71 & +10:44:52.4 & 12.73 & 1.00 & -10.71 & 2.20 & & 1.11 & LAMOST \\
57 & 04:49:17.88 & +10:39:53.0 & 10.59 & 0.99 & -20.01 & 2.20 & & 1.06 & Gaia DR3 \\
58 & 04:49:20.51 & +11:17:24.5 & 12.27 & 1.00 & -14.90 & 1.70 & & 1.08 & LAMOST \\
59 & 04:49:24.94 & +11:23:47.5 & 12.88 & 1.00 & -10.48 & 1.17 & & 0.93 & LAMOST \\
60 & 04:49:25.99 & +10:51:41.1 & 10.65 & 0.99 & -16.40 & 2.82 & & 1.00 & Gaia DR3 \\
61 & 04:49:26.27 & +10:41:12.6 & 11.47 & 1.00 & -9.73 & 1.91 & & 1.28 & Gaia DR3 \\
62 & 04:49:27.57 & +10:38:56.8 & 13.75 & 0.99 & -14.26 & 3.71 & & 0.99 & Gaia DR3 \\
63 & 04:49:28.46 & +10:40:19.2 & 11.69 & 0.99 & -15.53 & 2.86 & & 1.30 & Gaia DR3 \\
64 & 04:49:31.03 & +10:44:13.8 & 12.34 & 1.00 & -14.99 & 1.67 & & 1.10 & LAMOST \\
65 & 04:49:33.12 & +11:27:23.6 & 14.41 & 1.00 & -6.29 & 1.92 & & 0.97 & LAMOST \\
66 & 04:49:38.31 & +10:42:22.4 & 11.79 & 0.99 & -11.19 & 1.74 & & 1.12 & Gaia DR3 \\
67 & 04:49:39.59 & +10:37:41.5 & 14.00 & 0.98 & -13.64 & 3.43 & & 1.01 & Gaia DR3 \\
68 & 04:49:48.72 & +10:45:28.7 & 10.07 & 0.99 & -17.21 & 2.11 & & 1.07 & Gaia DR3 \\
69 & 04:50:16.99 & +11:50:43.9 & 13.93 & 1.00 & -12.63 & 2.82 & & 1.32 & LAMOST \\
70 & 04:50:31.50 & +10:58:52.5 & 9.54 & 0.98 & -18.75 & 1.49 & & 0.98 & Gaia DR3 \\
71 & 04:50:43.24 & +10:13:57.1 & 14.28 & 0.91 & -10.33 & 3.86 & & 1.01 & Gaia DR3 \\
72 & 04:50:43.77 & +10:44:36.7 & 12.79 & 1.00 & -12.00 & 2.73 & & 1.05 & Gaia DR3 \\
73 & 04:50:45.36 & +11:06:24.1 & 13.50 & 0.98 & -11.85 & 2.52 & & 1.04 & Gaia DR3 \\
74 & 04:50:50.39 & +10:59:09.8 & 14.30 & 0.98 & -14.62 & 3.83 & & 1.06 & Gaia DR3 \\
75 & 04:50:55.70 & +10:44:59.7 & 13.85 & 1.00 & -12.41 & 2.64 & & 1.07 & LAMOST \\
76 & 04:50:56.59 & +10:31:05.8 & 14.23 & 0.96 & -10.32 & 2.54 & & 1.03 & Gaia DR3 \\
77 & 04:51:18.71 & +11:52:38.0 & 14.46 & 0.62 & -11.80 & 5.79 & & 0.99 & Gaia DR3 \\
78 & 04:51:20.55 & +11:04:04.6 & 14.65 & 0.97 & -8.35 & 3.76 & & 1.02 & Gaia DR3 \\
\hline
\end{tabular}
\label{tab:NGC_1662}
\end{table*}

% Tablo: NGC_1778
\begin{table*} \footnotesize
\centering
\caption{Radial velocity measurements for NGC 1778}
\begin{tabular}{l c c c c c c c c l}
\hline\hline
ID & $\alpha$ (hh:mm:ss) & $\delta$ (dd:mm:ss) & $G$ (mag) & $P$ & $V_R$ (km s$^{-1}$)& $\sigma_{V_R}$ & & RUWE & Survey \\
\hline
1 & 05:07:00.89 & +37:04:34.3 & 14.33 & 0.97 & -14.41 & 2.09 & & 1.03 & Gaia DR3 \\
2 & 05:07:02.46 & +36:55:26.5 & 14.74 & 0.92 & -15.06 & 2.58 & & 1.03 & Gaia DR3 \\
3 & 05:07:48.17 & +37:13:50.3 & 11.85 & 0.99 & -16.85 & 18.42 & & 1.35 & Gaia DR3 \\
4 & 05:07:55.72 & +37:19:57.9 & 11.97 & 1.00 & 42.25 & 0.22 & & 1.12 & Gaia DR3 \\
5 & 05:07:59.79 & +37:02:12.3 & 11.61 & 1.00 & 24.61 & 16.90 & & 1.29 & Gaia DR3 \\
6 & 05:08:01.30 & +36:59:18.0 & 11.64 & 1.00 & 6.44 & 9.51 & & 1.25 & Gaia DR3 \\
7 & 05:08:03.50 & +37:10:33.2 & 14.78 & 0.99 & 0.59 & 7.83 & & 1.04 & Gaia DR3 \\
8 & 05:08:03.88 & +36:57:36.7 & 9.43 & 0.99 & 4.89 & 0.63 & & 1.35 & Gaia DR3 \\
9 & 05:08:15.54 & +37:02:47.3 & 14.44 & 1.00 & 7.21 & 21.87 & & 1.02 & Gaia DR3 \\
10 & 05:08:20.29 & +37:06:24.3 & 10.77 & 1.00 & -26.11 & 0.19 & & 0.92 & Gaia DR3 \\
11 & 05:08:21.75 & +37:06:42.4 & 11.54 & 1.00 & -6.21 & 24.85 & & 1.40 & Gaia DR3 \\
12 & 05:08:43.35 & +36:54:20.9 & 12.36 & 0.99 & 20.39 & 25.90 & & 0.94 & Gaia DR3 \\
13 & 05:08:49.56 & +37:01:25.9 & 12.22 & 1.00 & 11.10 & 22.20 & & 1.06 & Gaia DR3 \\
14 & 05:09:34.89 & +36:52:19.0 & 12.87 & 1.00 & -77.09 & 0.44 & & 0.97 & LAMOST \\
15 & 05:09:37.66 & +36:54:46.5 & 14.18 & 1.00 & -63.22 & 1.44 & & 1.11 & LAMOST \\
16 & 05:09:58.65 & +36:39:45.9 & 14.60 & 1.00 & -39.35 & 2.55 & & 1.08 & LAMOST \\
\hline
\end{tabular}
\label{tab:NGC_1778}
\end{table*}

% Tablo: NGC_2422
\begin{table*} \footnotesize
\centering
\caption{Radial velocity measurements for NGC 2422}
\begin{tabular}{l c c c c c c c c l}
\hline\hline
ID & $\alpha$ (hh:mm:ss) & $\delta$ (dd:mm:ss) & $G$ (mag) & $P$ & $V_R$ (km s$^{-1}$)& $\sigma_{V_R}$ & & RUWE & Survey \\
\hline
1 & 07:32:11.90 & -14:08:20.8 & 14.84 & 0.80 & -43.28 & 8.04 & & 0.95 & Gaia DR3 \\
2 & 07:32:52.49 & -13:41:58.4 & 10.57 & 0.80 & 28.17 & 3.16 & & 0.91 & Gaia DR3 \\
3 & 07:32:56.34 & -14:50:24.9 & 10.59 & 0.97 & 24.80 & 4.06 & & 1.03 & Gaia DR3 \\
4 & 07:33:07.88 & -15:10:42.2 & 9.26 & 0.54 & 42.93 & 5.68 & & 1.00 & Gaia DR3 \\
5 & 07:33:16.99 & -14:22:59.6 & 12.01 & 1.00 & 50.10 & 1.00 & & 0.93 & Gaia DR3 \\
6 & 07:33:26.43 & -13:48:38.2 & 10.57 & 0.93 & 33.11 & 1.95 & & 0.89 & Gaia DR3 \\
7 & 07:33:38.68 & -14:33:18.4 & 14.00 & 0.95 & 35.00 & 3.87 & & 1.02 & Gaia DR3 \\
8 & 07:33:47.23 & -15:20:14.2 & 14.71 & 0.53 & 29.22 & 6.15 & & 0.96 & Gaia DR3 \\
9 & 07:33:52.33 & -13:50:20.8 & 12.38 & 1.00 & 36.97 & 2.42 & & 0.92 & Gaia DR3 \\
10 & 07:33:56.28 & -15:03:42.9 & 10.88 & 0.64 & 33.77 & 4.14 & & 1.04 & Gaia DR3 \\
11 & 07:34:07.17 & -14:34:42.1 & 11.74 & 0.99 & 33.59 & 1.11 & & 1.27 & Gaia DR3 \\
12 & 07:34:10.58 & -14:42:57.4 & 13.86 & 0.99 & 34.51 & 3.46 & & 1.02 & Gaia DR3 \\
13 & 07:34:19.60 & -14:14:19.7 & 14.96 & 0.99 & 14.62 & 15.13 & & 0.99 & Gaia DR3 \\
14 & 07:34:22.27 & -14:08:41.6 & 12.29 & 1.00 & 35.83 & 3.44 & & 0.92 & Gaia DR3 \\
15 & 07:34:22.30 & -13:51:55.9 & 14.43 & 0.98 & 34.17 & 4.91 & & 1.01 & Gaia DR3 \\
16 & 07:34:39.77 & -13:58:11.2 & 14.43 & 0.95 & 30.13 & 3.89 & & 1.01 & Gaia DR3 \\
17 & 07:34:41.90 & -13:59:14.5 & 12.09 & 1.00 & 18.07 & 6.14 & & 1.28 & Gaia DR3 \\
18 & 07:34:45.40 & -15:06:33.4 & 14.67 & 0.98 & 36.71 & 4.52 & & 1.09 & Gaia DR3 \\
19 & 07:34:45.51 & -14:19:18.6 & 12.66 & 0.94 & -2.43 & 35.40 & & 0.93 & Gaia DR3 \\
20 & 07:34:47.41 & -13:58:33.5 & 10.26 & 0.98 & 33.24 & 0.85 & & 1.01 & Gaia DR3 \\
21 & 07:34:56.28 & -14:21:56.2 & 11.71 & 1.00 & 35.77 & 1.16 & & 0.87 & Gaia DR3 \\
22 & 07:35:02.96 & -15:34:34.6 & 13.17 & 0.82 & 32.24 & 3.36 & & 0.90 & Gaia DR3 \\
23 & 07:35:05.08 & -14:34:27.5 & 14.57 & 1.00 & 38.77 & 4.63 & & 1.12 & Gaia DR3 \\
24 & 07:35:05.31 & -14:02:41.1 & 9.89 & 0.99 & 32.61 & 0.77 & & 0.93 & Gaia DR3 \\
25 & 07:35:13.02 & -14:48:11.3 & 12.53 & 1.00 & 34.10 & 5.01 & & 0.97 & Gaia DR3 \\
26 & 07:35:16.22 & -14:42:53.6 & 10.92 & 1.00 & 40.11 & 2.04 & & 0.89 & RAVE \\
27 & 07:35:17.58 & -15:05:46.6 & 14.51 & 0.99 & 28.36 & 5.47 & & 1.03 & Gaia DR3 \\
28 & 07:35:18.10 & -14:48:31.0 & 14.14 & 1.00 & 36.16 & 3.52 & & 0.99 & Gaia DR3 \\
29 & 07:35:18.84 & -14:39:44.3 & 14.30 & 1.00 & 39.93 & 4.28 & & 1.00 & Gaia DR3 \\
30 & 07:35:19.53 & -14:07:17.7 & 11.33 & 1.00 & 36.10 & 1.20 & & 1.05 & Gaia DR3 \\
31 & 07:35:19.61 & -14:59:14.5 & 13.22 & 0.99 & 37.27 & 2.86 & & 0.95 & Gaia DR3 \\
32 & 07:35:22.38 & -13:18:00.2 & 12.79 & 1.00 & 36.99 & 3.19 & & 0.95 & Gaia DR3 \\
33 & 07:35:23.88 & -14:46:52.6 & 14.65 & 0.99 & 39.05 & 4.70 & & 0.98 & Gaia DR3 \\
34 & 07:35:28.44 & -15:37:30.2 & 14.28 & 0.73 & 42.74 & 3.70 & & 1.02 & Gaia DR3 \\
35 & 07:35:30.91 & -14:29:22.0 & 12.16 & 1.00 & 31.83 & 2.45 & & 0.89 & Gaia DR3 \\
36 & 07:35:31.48 & -14:36:22.6 & 14.91 & 0.99 & 44.62 & 6.76 & & 1.01 & Gaia DR3 \\
37 & 07:35:31.54 & -13:33:19.3 & 13.33 & 0.96 & 36.21 & 2.93 & & 0.96 & Gaia DR3 \\
38 & 07:35:31.67 & -14:27:10.6 & 10.08 & 1.00 & 30.17 & 6.31 & & 0.83 & Gaia DR3 \\
39 & 07:35:32.26 & -14:34:01.8 & 11.29 & 1.00 & 35.24 & 1.79 & & 1.04 & Gaia DR3 \\
40 & 07:35:33.54 & -14:22:11.7 & 14.36 & 1.00 & 34.79 & 3.95 & & 1.06 & Gaia DR3 \\
41 & 07:35:36.28 & -14:40:13.9 & 8.80 & 1.00 & 37.27 & 1.86 & & 1.08 & Gaia DR3 \\
42 & 07:35:39.10 & -14:02:33.1 & 11.39 & 1.00 & 39.60 & 2.04 & & 1.02 & RAVE \\
43 & 07:35:39.17 & -14:29:48.6 & 14.43 & 1.00 & 37.47 & 5.75 & & 0.91 & Gaia DR3 \\
44 & 07:35:41.48 & -14:37:30.2 & 14.78 & 1.00 & 35.66 & 6.04 & & 0.96 & Gaia DR3 \\
45 & 07:35:44.00 & -13:18:00.0 & 11.96 & 1.00 & 39.00 & 10.82 & & 0.89 & Gaia DR3 \\
46 & 07:35:47.11 & -14:10:28.0 & 11.26 & 1.00 & 44.06 & 4.45 & & 0.98 & Gaia DR3 \\
47 & 07:35:47.28 & -14:30:41.2 & 13.07 & 1.00 & 33.87 & 3.17 & & 1.05 & Gaia DR3 \\
48 & 07:35:47.39 & -14:19:00.0 & 14.84 & 1.00 & 40.34 & 4.55 & & 1.02 & Gaia DR3 \\
49 & 07:35:49.28 & -14:22:26.1 & 13.27 & 0.99 & 31.72 & 4.34 & & 1.10 & Gaia DR3 \\
50 & 07:35:49.59 & -14:57:00.8 & 14.89 & 0.97 & 43.00 & 3.99 & & 0.94 & Gaia DR3 \\
51 & 07:35:50.30 & -15:10:52.1 & 12.44 & 1.00 & 21.30 & 4.20 & & 0.84 & Gaia DR3 \\
52 & 07:35:50.57 & -14:57:53.0 & 12.11 & 1.00 & 37.51 & 2.76 & & 0.91 & Gaia DR3 \\
53 & 07:35:50.77 & -14:37:49.5 & 12.82 & 1.00 & 33.31 & 1.20 & & 1.05 & Gaia DR3 \\
54 & 07:35:50.85 & -14:11:18.3 & 12.54 & 1.00 & 41.46 & 4.63 & & 0.93 & Gaia DR3 \\
55 & 07:35:53.15 & -14:26:41.5 & 11.57 & 1.00 & 37.48 & 1.34 & & 0.91 & Gaia DR3 \\
56 & 07:35:53.22 & -14:35:30.3 & 10.71 & 1.00 & 12.29 & 9.95 & & 1.16 & Gaia DR3 \\
57 & 07:35:54.38 & -14:21:09.1 & 13.59 & 1.00 & 32.84 & 3.07 & & 1.01 & Gaia DR3 \\
58 & 07:35:54.67 & -14:44:37.4 & 13.10 & 1.00 & 33.00 & 2.38 & & 1.04 & Gaia DR3 \\
59 & 07:35:54.95 & -14:52:34.6 & 14.71 & 1.00 & 29.94 & 5.08 & & 1.02 & Gaia DR3 \\
60 & 07:35:56.96 & -14:42:39.0 & 7.93 & 1.00 & 44.46 & 1.08 & & 0.93 & Gaia DR3 \\
61 & 07:35:57.52 & -14:32:40.7 & 12.26 & 1.00 & -8.83 & 10.31 & & 1.11 & Gaia DR3 \\
62 & 07:35:57.69 & -14:16:26.2 & 11.04 & 1.00 & 35.94 & 3.00 & & 1.31 & Gaia DR3 \\
63 & 07:35:58.20 & -14:14:24.0 & 13.50 & 1.00 & 33.41 & 3.35 & & 1.35 & Gaia DR3 \\
64 & 07:35:59.77 & -15:00:05.7 & 13.82 & 1.00 & 23.67 & 5.66 & & 0.97 & Gaia DR3 \\
65 & 07:36:01.64 & -14:19:23.0 & 14.53 & 1.00 & 34.50 & 4.98 & & 1.04 & Gaia DR3 \\
66 & 07:36:04.70 & -14:29:18.1 & 9.78 & 1.00 & 22.44 & 6.50 & & 0.82 & Gaia DR3 \\
67 & 07:36:05.38 & -14:38:22.9 & 13.29 & 1.00 & 32.33 & 4.21 & & 1.15 & Gaia DR3 \\
68 & 07:36:08.08 & -14:29:42.1 & 12.57 & 1.00 & 33.88 & 2.58 & & 1.30 & Gaia DR3 \\
69 & 07:36:08.88 & -14:30:36.8 & 12.25 & 1.00 & 37.72 & 2.22 & & 0.91 & Gaia DR3 \\
70 & 07:36:09.88 & -14:40:17.4 & 10.49 & 1.00 & 33.69 & 4.73 & & 0.97 & Gaia DR3 \\
71 & 07:36:10.70 & -14:50:44.0 & 14.39 & 1.00 & 40.52 & 5.49 & & 1.08 & Gaia DR3 \\
72 & 07:36:10.71 & -14:27:40.9 & 9.88 & 1.00 & 30.13 & 4.09 & & 0.91 & Gaia DR3 \\
73 & 07:36:10.78 & -14:22:48.8 & 9.96 & 1.00 & 31.84 & 3.84 & & 0.84 & Gaia DR3 \\
74 & 07:36:10.98 & -15:04:45.6 & 14.57 & 0.99 & 61.92 & 10.58 & & 1.04 & Gaia DR3 \\
75 & 07:36:11.76 & -14:37:16.9 & 13.57 & 1.00 & 38.87 & 2.84 & & 1.11 & Gaia DR3 \\
76 & 07:36:12.17 & -14:38:02.4 & 10.96 & 1.00 & 36.42 & 2.45 & & 1.17 & RAVE \\
77 & 07:36:12.17 & -14:26:38.5 & 13.65 & 1.00 & 37.27 & 4.04 & & 1.03 & Gaia DR3 \\
78 & 07:36:12.98 & -14:52:18.6 & 14.21 & 1.00 & 35.92 & 3.48 & & 1.02 & Gaia DR3 \\
79 & 07:36:14.18 & -14:23:46.7 & 11.97 & 1.00 & 30.42 & 2.73 & & 1.24 & Gaia DR3 \\
80 & 07:36:14.37 & -14:40:27.6 & 12.87 & 1.00 & 32.27 & 2.82 & & 1.13 & Gaia DR3 \\
81 & 07:36:14.61 & -14:34:11.3 & 10.70 & 1.00 & 34.10 & 2.28 & & 1.05 & Gaia DR3 \\
82 & 07:36:14.64 & -14:20:49.4 & 13.80 & 1.00 & 37.81 & 3.42 & & 0.97 & Gaia DR3 \\
83 & 07:36:15.22 & -14:35:43.2 & 11.63 & 1.00 & 37.91 & 0.98 & & 0.91 & Gaia DR3 \\
84 & 07:36:15.53 & -14:22:22.5 & 13.66 & 1.00 & 30.97 & 4.00 & & 1.04 & Gaia DR3 \\
85 & 07:36:17.88 & -13:48:37.1 & 14.58 & 0.99 & 33.92 & 4.82 & & 1.07 & Gaia DR3 \\
86 & 07:36:17.93 & -14:55:40.6 & 13.10 & 1.00 & 35.74 & 5.59 & & 1.04 & Gaia DR3 \\
87 & 07:36:17.96 & -13:19:13.9 & 9.76 & 0.60 & 24.08 & 3.27 & & 1.00 & Gaia DR3 \\
88 & 07:36:18.18 & -14:15:42.6 & 14.77 & 1.00 & 37.99 & 11.73 & & 1.08 & Gaia DR3 \\
89 & 07:36:18.60 & -14:22:59.8 & 12.96 & 1.00 & 31.65 & 2.56 & & 1.02 & Gaia DR3 \\
90 & 07:36:20.26 & -14:20:24.2 & 12.97 & 1.00 & 40.34 & 4.09 & & 1.12 & Gaia DR3 \\
91 & 07:36:20.30 & -15:11:22.1 & 13.86 & 0.99 & 30.68 & 3.32 & & 0.98 & Gaia DR3 \\
92 & 07:36:21.35 & -14:26:30.3 & 13.77 & 1.00 & 27.10 & 4.65 & & 1.08 & Gaia DR3 \\
93 & 07:36:21.64 & -14:44:26.6 & 9.11 & 1.00 & 29.67 & 3.45 & & 0.98 & Gaia DR3 \\
94 & 07:36:22.06 & -14:30:28.3 & 10.41 & 1.00 & 30.60 & 2.70 & & 0.88 & Gaia DR3 \\
95 & 07:36:22.62 & -14:29:45.5 & 8.70 & 1.00 & 37.98 & 2.59 & & 0.91 & Gaia DR3 \\
96 & 07:36:22.72 & -14:23:32.0 & 14.51 & 1.00 & 32.43 & 6.74 & & 0.96 & Gaia DR3 \\
97 & 07:36:24.35 & -14:39:57.0 & 12.54 & 1.00 & 36.56 & 12.04 & & 0.95 & Gaia DR3 \\
98 & 07:36:24.90 & -14:27:14.3 & 14.92 & 1.00 & 27.34 & 6.81 & & 1.02 & Gaia DR3 \\
99 & 07:36:25.15 & -14:32:30.2 & 12.59 & 1.00 & 37.06 & 2.16 & & 1.17 & Gaia DR3 \\
100 & 07:36:25.16 & -14:54:36.6 & 13.89 & 0.99 & 36.21 & 5.11 & & 1.10 & Gaia DR3 \\
101 & 07:36:25.23 & -14:34:35.4 & 14.84 & 1.00 & 82.16 & 8.88 & & 1.38 & Gaia DR3 \\
102 & 07:36:25.35 & -13:22:18.2 & 11.35 & 1.00 & 35.96 & 3.51 & & 1.23 & Gaia DR3 \\
103 & 07:36:25.64 & -14:11:06.4 & 14.68 & 1.00 & 29.55 & 5.54 & & 1.04 & Gaia DR3 \\
104 & 07:36:25.79 & -13:56:29.1 & 14.84 & 1.00 & 32.35 & 7.76 & & 1.00 & Gaia DR3 \\
105 & 07:36:25.79 & -14:29:07.7 & 9.43 & 1.00 & 29.14 & 5.44 & & 0.89 & Gaia DR3 \\
106 & 07:36:26.15 & -14:39:29.9 & 12.56 & 1.00 & 35.71 & 3.83 & & 0.97 & Gaia DR3 \\
107 & 07:36:27.46 & -14:38:47.2 & 11.78 & 1.00 & 30.51 & 6.06 & & 0.93 & Gaia DR3 \\
108 & 07:36:27.58 & -14:13:36.7 & 9.93 & 1.00 & 28.52 & 4.43 & & 0.82 & Gaia DR3 \\
109 & 07:36:28.53 & -14:56:54.4 & 14.78 & 1.00 & 90.66 & 8.42 & & 0.96 & Gaia DR3 \\
110 & 07:36:30.01 & -14:19:31.2 & 11.58 & 1.00 & 35.95 & 2.08 & & 0.86 & Gaia DR3 \\
111 & 07:36:31.36 & -14:00:21.1 & 11.12 & 0.99 & 35.82 & 1.48 & & 1.09 & Gaia DR3 \\
112 & 07:36:31.85 & -14:29:41.8 & 10.76 & 1.00 & 27.82 & 2.95 & & 0.97 & Gaia DR3 \\
113 & 07:36:32.11 & -14:28:04.5 & 11.41 & 1.00 & 36.60 & 10.57 & & 0.86 & Gaia DR3 \\
114 & 07:36:32.78 & -14:14:33.4 & 8.64 & 1.00 & 32.22 & 1.69 & & 0.85 & Gaia DR3 \\
115 & 07:36:34.88 & -14:25:49.0 & 8.77 & 1.00 & 34.45 & 2.29 & & 0.91 & Gaia DR3 \\
116 & 07:36:35.70 & -14:29:00.4 & 7.09 & 1.00 & 33.00 & 3.28 & & 1.00 & Gaia DR3 \\
117 & 07:36:36.00 & -14:32:37.8 & 11.49 & 1.00 & 39.53 & 2.58 & & 0.81 & Gaia DR3 \\
118 & 07:36:36.48 & -14:08:37.8 & 9.81 & 1.00 & 27.45 & 3.37 & & 0.93 & Gaia DR3 \\
119 & 07:36:37.04 & -14:30:51.7 & 12.31 & 1.00 & 29.77 & 3.94 & & 0.90 & Gaia DR3 \\
120 & 07:36:37.07 & -14:09:53.6 & 14.15 & 1.00 & 35.28 & 5.20 & & 0.98 & Gaia DR3 \\
121 & 07:36:37.63 & -14:42:13.0 & 12.67 & 1.00 & 34.55 & 4.75 & & 0.98 & Gaia DR3 \\
122 & 07:36:37.68 & -14:38:18.9 & 14.62 & 1.00 & 46.44 & 11.67 & & 1.03 & Gaia DR3 \\
123 & 07:36:38.15 & -14:41:29.3 & 13.15 & 1.00 & 38.00 & 3.35 & & 0.95 & Gaia DR3 \\
124 & 07:36:38.18 & -14:58:51.4 & 12.34 & 1.00 & 36.60 & 1.89 & & 0.87 & Gaia DR3 \\
125 & 07:36:38.64 & -14:24:48.8 & 11.65 & 1.00 & 37.08 & 2.30 & & 0.89 & Gaia DR3 \\
126 & 07:36:39.04 & -14:50:51.8 & 11.51 & 0.99 & 36.21 & 4.98 & & 0.97 & Gaia DR3 \\
127 & 07:36:39.13 & -14:37:30.8 & 12.93 & 1.00 & 34.80 & 2.35 & & 1.03 & Gaia DR3 \\
128 & 07:36:39.43 & -14:23:34.2 & 10.16 & 1.00 & 31.67 & 2.52 & & 0.81 & Gaia DR3 \\
129 & 07:36:39.54 & -14:39:14.3 & 13.68 & 1.00 & 34.22 & 2.89 & & 1.04 & Gaia DR3 \\
130 & 07:36:39.90 & -14:33:14.9 & 14.83 & 1.00 & 47.95 & 14.75 & & 1.04 & Gaia DR3 \\
131 & 07:36:40.51 & -14:29:14.8 & 9.71 & 1.00 & 37.81 & 1.89 & & 1.20 & Gaia DR3 \\
132 & 07:36:41.02 & -14:34:45.7 & 11.13 & 1.00 & 42.04 & 3.58 & & 1.02 & Gaia DR3 \\
133 & 07:36:41.25 & -14:26:37.0 & 6.67 & 1.00 & 50.24 & 3.28 & & 1.08 & Gaia DR3 \\
134 & 07:36:41.27 & -14:35:30.8 & 11.37 & 1.00 & 32.56 & 2.72 & & 0.92 & Gaia DR3 \\
135 & 07:36:42.18 & -14:32:31.1 & 11.18 & 1.00 & 29.40 & 5.11 & & 1.02 & Gaia DR3 \\
136 & 07:36:43.35 & -14:40:55.2 & 11.67 & 0.73 & 11.83 & 3.71 & & 0.99 & Gaia DR3 \\
137 & 07:36:43.74 & -14:28:46.7 & 11.64 & 1.00 & 35.90 & 1.32 & & 0.87 & Gaia DR3 \\
138 & 07:36:44.97 & -14:21:44.8 & 14.06 & 1.00 & 39.87 & 7.00 & & 0.99 & Gaia DR3 \\
139 & 07:36:45.64 & -14:28:55.3 & 12.83 & 1.00 & 31.78 & 2.85 & & 1.00 & Gaia DR3 \\
140 & 07:36:45.77 & -14:34:34.9 & 14.31 & 1.00 & 32.81 & 3.64 & & 1.01 & Gaia DR3 \\
141 & 07:36:45.80 & -15:27:45.5 & 11.36 & 1.00 & 34.04 & 3.47 & & 0.97 & Gaia DR3 \\
142 & 07:36:45.84 & -14:37:51.4 & 12.00 & 1.00 & 37.61 & 1.72 & & 0.95 & Gaia DR3 \\
143 & 07:36:46.43 & -14:21:38.8 & 13.55 & 1.00 & 34.81 & 2.47 & & 0.93 & Gaia DR3 \\
144 & 07:36:46.48 & -14:24:19.9 & 10.33 & 1.00 & 24.07 & 4.68 & & 0.96 & Gaia DR3 \\
145 & 07:36:48.62 & -14:22:25.0 & 13.90 & 1.00 & 34.05 & 4.79 & & 0.97 & Gaia DR3 \\
146 & 07:36:50.06 & -14:22:59.6 & 12.29 & 1.00 & 36.31 & 2.65 & & 0.94 & Gaia DR3 \\
147 & 07:36:51.10 & -13:24:37.0 & 12.28 & 1.00 & 36.70 & 5.08 & & 1.01 & Gaia DR3 \\
148 & 07:36:52.32 & -14:24:32.3 & 9.76 & 1.00 & 30.61 & 2.61 & & 0.93 & Gaia DR3 \\
149 & 07:36:52.57 & -14:58:34.6 & 12.49 & 1.00 & 33.48 & 4.06 & & 0.96 & Gaia DR3 \\
150 & 07:36:52.73 & -14:34:13.3 & 14.39 & 0.99 & 29.59 & 6.76 & & 1.04 & Gaia DR3 \\
151 & 07:36:53.05 & -14:33:15.7 & 10.11 & 1.00 & 23.48 & 3.31 & & 0.97 & Gaia DR3 \\
152 & 07:36:53.33 & -14:15:10.9 & 14.71 & 1.00 & 39.24 & 6.39 & & 1.04 & Gaia DR3 \\
153 & 07:36:53.88 & -14:23:30.1 & 14.59 & 1.00 & 78.66 & 8.83 & & 0.95 & Gaia DR3 \\
154 & 07:36:54.68 & -15:05:43.4 & 13.41 & 1.00 & 44.41 & 3.77 & & 1.00 & Gaia DR3 \\
155 & 07:36:54.90 & -14:30:29.9 & 13.10 & 1.00 & 33.98 & 2.97 & & 0.94 & Gaia DR3 \\
156 & 07:36:55.22 & -15:17:34.2 & 13.16 & 0.99 & 37.63 & 4.32 & & 0.98 & Gaia DR3 \\
157 & 07:36:55.25 & -14:33:17.6 & 10.68 & 0.99 & 33.45 & 1.10 & & 1.11 & Gaia DR3 \\
158 & 07:36:56.63 & -14:27:42.6 & 13.83 & 1.00 & 36.51 & 3.54 & & 0.97 & Gaia DR3 \\
159 & 07:36:57.57 & -14:50:44.6 & 13.43 & 1.00 & 36.61 & 3.62 & & 1.01 & Gaia DR3 \\
160 & 07:36:58.40 & -14:35:54.4 & 13.33 & 1.00 & 32.92 & 2.76 & & 0.95 & Gaia DR3 \\
161 & 07:36:58.61 & -14:29:54.2 & 14.36 & 0.99 & 34.24 & 4.64 & & 1.05 & Gaia DR3 \\
162 & 07:36:58.85 & -14:36:21.8 & 12.32 & 1.00 & 36.82 & 2.35 & & 1.00 & Gaia DR3 \\
163 & 07:36:59.02 & -13:56:16.9 & 12.15 & 1.00 & 37.56 & 5.44 & & 0.99 & Gaia DR3 \\
164 & 07:36:59.59 & -14:55:53.2 & 14.54 & 1.00 & 31.52 & 6.94 & & 1.02 & Gaia DR3 \\
165 & 07:37:00.32 & -14:26:03.3 & 13.17 & 1.00 & 40.14 & 2.65 & & 0.97 & Gaia DR3 \\
166 & 07:37:01.01 & -14:39:34.4 & 11.16 & 1.00 & 35.52 & 1.19 & & 0.89 & Gaia DR3 \\
167 & 07:37:02.36 & -14:31:13.6 & 11.09 & 1.00 & 36.68 & 1.46 & & 0.89 & Gaia DR3 \\
168 & 07:37:03.97 & -15:19:23.5 & 10.19 & 0.94 & 26.96 & 3.32 & & 1.03 & Gaia DR3 \\
169 & 07:37:04.89 & -14:45:24.2 & 14.80 & 0.99 & 38.69 & 5.37 & & 1.01 & Gaia DR3 \\
170 & 07:37:05.66 & -14:24:24.5 & 10.32 & 1.00 & 22.31 & 5.68 & & 0.86 & Gaia DR3 \\
171 & 07:37:06.63 & -14:31:45.6 & 12.39 & 1.00 & 38.48 & 12.46 & & 0.95 & Gaia DR3 \\
172 & 07:37:07.17 & -14:15:42.5 & 12.36 & 1.00 & 37.29 & 29.21 & & 0.91 & Gaia DR3 \\
173 & 07:37:08.00 & -14:04:16.7 & 14.61 & 1.00 & 35.89 & 14.19 & & 1.20 & Gaia DR3 \\
174 & 07:37:08.26 & -14:33:14.7 & 10.48 & 1.00 & 30.71 & 1.32 & & 1.34 & RAVE \\
175 & 07:37:09.83 & -14:24:54.3 & 15.01 & 0.97 & 71.09 & 11.35 & & 1.08 & Gaia DR3 \\
176 & 07:37:10.52 & -14:33:41.5 & 11.70 & 1.00 & 40.52 & 3.35 & & 0.89 & Gaia DR3 \\
177 & 07:37:11.38 & -14:15:57.5 & 11.41 & 1.00 & 35.31 & 2.15 & & 0.94 & Gaia DR3 \\
178 & 07:37:13.11 & -14:29:11.8 & 11.26 & 1.00 & 33.65 & 1.31 & & 0.99 & Gaia DR3 \\
179 & 07:37:14.50 & -14:25:18.0 & 9.95 & 1.00 & 29.51 & 4.60 & & 0.94 & Gaia DR3 \\
180 & 07:37:14.82 & -14:32:14.9 & 12.06 & 1.00 & 37.33 & 4.00 & & 0.89 & Gaia DR3 \\
181 & 07:37:15.28 & -14:25:56.7 & 11.91 & 1.00 & 26.30 & 4.12 & & 0.99 & Gaia DR3 \\
182 & 07:37:15.40 & -14:33:35.6 & 13.32 & 1.00 & 31.86 & 6.25 & & 1.00 & Gaia DR3 \\
183 & 07:37:15.56 & -14:31:48.8 & 12.40 & 1.00 & 31.79 & 3.55 & & 1.03 & Gaia DR3 \\
184 & 07:37:18.22 & -14:32:45.7 & 14.93 & 1.00 & 24.60 & 8.43 & & 0.96 & Gaia DR3 \\
185 & 07:37:22.30 & -14:29:41.4 & 14.82 & 1.00 & 38.57 & 6.72 & & 1.30 & Gaia DR3 \\
186 & 07:37:22.52 & -14:35:49.7 & 10.72 & 1.00 & 18.43 & 5.78 & & 0.99 & RAVE \\
187 & 07:37:23.29 & -14:25:11.6 & 12.94 & 1.00 & 35.84 & 2.18 & & 0.94 & Gaia DR3 \\
188 & 07:37:24.69 & -14:23:36.7 & 11.94 & 1.00 & 34.40 & 6.47 & & 0.97 & Gaia DR3 \\
189 & 07:37:27.21 & -14:17:12.9 & 14.36 & 0.99 & -5.14 & 5.94 & & 0.96 & Gaia DR3 \\
190 & 07:37:27.91 & -14:25:17.6 & 12.89 & 1.00 & 33.18 & 2.38 & & 1.04 & Gaia DR3 \\
191 & 07:37:31.09 & -14:18:00.1 & 12.71 & 1.00 & 32.40 & 5.38 & & 1.02 & Gaia DR3 \\
192 & 07:37:32.91 & -14:29:19.4 & 14.79 & 1.00 & 41.03 & 6.76 & & 1.00 & Gaia DR3 \\
193 & 07:37:34.84 & -14:24:29.4 & 11.64 & 1.00 & 39.13 & 2.84 & & 0.99 & Gaia DR3 \\
194 & 07:37:35.05 & -14:04:26.3 & 13.97 & 1.00 & 30.80 & 4.18 & & 0.97 & Gaia DR3 \\
195 & 07:37:37.11 & -14:25:25.5 & 8.90 & 1.00 & 31.42 & 2.98 & & 0.85 & Gaia DR3 \\
196 & 07:37:37.73 & -14:27:49.8 & 10.92 & 1.00 & 30.44 & 3.32 & & 1.27 & RAVE \\
197 & 07:37:38.80 & -14:26:26.7 & 6.49 & 1.00 & 69.56 & 0.66 & & 0.96 & Gaia DR3 \\
198 & 07:37:38.99 & -14:40:05.2 & 13.44 & 1.00 & 27.43 & 5.23 & & 1.05 & Gaia DR3 \\
199 & 07:37:39.18 & -14:02:02.6 & 10.51 & 1.00 & 33.30 & 1.08 & & 0.96 & Gaia DR3 \\
200 & 07:37:43.01 & -13:55:25.5 & 11.73 & 1.00 & 38.38 & 6.72 & & 0.95 & Gaia DR3 \\
201 & 07:37:45.81 & -14:35:47.7 & 10.72 & 1.00 & 28.35 & 7.08 & & 0.94 & Gaia DR3 \\
202 & 07:37:46.02 & -13:40:13.0 & 11.81 & 1.00 & 25.47 & 9.17 & & 0.97 & Gaia DR3 \\
203 & 07:37:46.32 & -14:36:38.8 & 14.24 & 1.00 & 9.25 & 5.14 & & 1.10 & Gaia DR3 \\
204 & 07:37:47.34 & -14:15:39.7 & 14.69 & 1.00 & 33.71 & 8.40 & & 1.04 & Gaia DR3 \\
205 & 07:37:48.62 & -14:30:29.1 & 11.67 & 1.00 & 37.01 & 1.01 & & 1.04 & Gaia DR3 \\
206 & 07:37:58.26 & -14:21:49.0 & 14.09 & 1.00 & 37.44 & 4.50 & & 0.99 & Gaia DR3 \\
207 & 07:37:58.94 & -15:05:45.4 & 13.27 & 0.99 & 34.54 & 2.62 & & 1.01 & Gaia DR3 \\
208 & 07:37:59.99 & -14:48:18.0 & 13.37 & 1.00 & 38.08 & 6.43 & & 0.95 & Gaia DR3 \\
209 & 07:38:01.11 & -13:43:34.5 & 10.01 & 0.98 & 23.01 & 4.25 & & 0.88 & Gaia DR3 \\
210 & 07:38:03.84 & -13:44:04.6 & 10.09 & 0.83 & 27.05 & 2.47 & & 0.95 & Gaia DR3 \\
211 & 07:38:05.72 & -15:06:17.8 & 14.30 & 0.99 & 33.22 & 4.38 & & 0.97 & Gaia DR3 \\
212 & 07:38:07.82 & -14:12:09.8 & 14.96 & 1.00 & 16.05 & 9.96 & & 1.00 & Gaia DR3 \\
213 & 07:38:13.75 & -14:14:24.7 & 13.71 & 0.98 & 33.94 & 5.73 & & 1.04 & Gaia DR3 \\
214 & 07:38:14.46 & -14:26:55.1 & 13.79 & 1.00 & 33.94 & 2.77 & & 1.01 & Gaia DR3 \\
215 & 07:38:14.60 & -14:04:59.0 & 10.95 & 1.00 & 34.53 & 8.25 & & 1.26 & Gaia DR3 \\
216 & 07:38:24.83 & -14:18:49.2 & 12.47 & 1.00 & 25.66 & 4.60 & & 0.91 & Gaia DR3 \\
217 & 07:38:26.53 & -14:21:04.1 & 14.42 & 1.00 & 35.59 & 4.38 & & 1.01 & Gaia DR3 \\
218 & 07:38:31.42 & -14:35:42.0 & 12.09 & 1.00 & 35.86 & 0.80 & & 0.91 & Gaia DR3 \\
219 & 07:38:35.64 & -14:29:53.9 & 11.03 & 1.00 & 34.67 & 5.48 & & 0.99 & RAVE \\
220 & 07:38:42.44 & -14:24:16.6 & 12.68 & 0.99 & 34.18 & 4.67 & & 0.90 & Gaia DR3 \\
221 & 07:38:55.93 & -14:55:42.6 & 14.02 & 0.99 & 44.45 & 4.76 & & 1.01 & Gaia DR3 \\
222 & 07:39:03.66 & -14:13:46.9 & 12.88 & 0.99 & 38.92 & 3.41 & & 0.92 & Gaia DR3 \\
223 & 07:39:17.78 & -14:20:45.4 & 14.62 & 0.98 & 32.82 & 4.71 & & 1.03 & Gaia DR3 \\
224 & 07:39:20.99 & -13:26:44.5 & 9.69 & 0.63 & 21.64 & 16.04 & & 1.04 & Gaia DR3 \\
225 & 07:39:25.52 & -15:06:48.3 & 10.80 & 0.97 & 22.98 & 6.33 & & 1.12 & Gaia DR3 \\
226 & 07:39:32.92 & -13:59:10.9 & 14.14 & 0.98 & 34.99 & 6.11 & & 0.97 & Gaia DR3 \\
227 & 07:39:34.08 & -14:09:06.1 & 9.36 & 0.99 & 31.23 & 3.52 & & 1.03 & Gaia DR3 \\
228 & 07:39:37.11 & -14:51:41.5 & 14.68 & 0.97 & 29.44 & 5.41 & & 0.97 & Gaia DR3 \\
229 & 07:39:57.15 & -13:50:46.6 & 13.11 & 1.00 & 36.18 & 2.20 & & 0.96 & Gaia DR3 \\
230 & 07:40:46.53 & -14:30:48.2 & 9.90 & 0.88 & 19.31 & 4.90 & & 0.92 & Gaia DR3 \\
231 & 07:41:03.37 & -14:34:07.2 & 10.14 & 0.73 & 30.82 & 6.03 & & 0.93 & Gaia DR3 \\
\hline
\end{tabular}
\label{tab:NGC_2422}
\end{table*}


% Tablo: NGC_2437
\begin{table*} \footnotesize
\centering
\caption{Radial velocity measurements for NGC 2437}
\begin{tabular}{l c c c c c c c c l}
\hline\hline
ID & $\alpha$ (hh:mm:ss) & $\delta$ (dd:mm:ss) & $G$ (mag) & $P$ & $V_R$ (km s$^{-1}$)& $\sigma_{V_R}$ & & RUWE & Survey \\
\hline
1 & 07:39:36.19 & -14:40:19.3 & 14.40 & 0.73 & 71.66 & 28.70 & & 1.09 & Gaia DR3 \\
2 & 07:39:57.78 & -14:51:27.5 & 11.24 & 0.87 & 50.42 & 6.39 & & 0.95 & Gaia DR3 \\
3 & 07:40:22.56 & -14:39:06.3 & 11.77 & 1.00 & 33.70 & 6.71 & & 0.94 & Gaia DR3 \\
4 & 07:40:25.60 & -14:22:08.2 & 14.13 & 0.66 & 47.90 & 14.69 & & 1.01 & Gaia DR3 \\
5 & 07:40:26.09 & -14:48:00.7 & 11.71 & 0.91 & 46.57 & 11.08 & & 0.88 & Gaia DR3 \\
6 & 07:40:28.33 & -14:48:52.6 & 14.73 & 0.95 & 46.18 & 8.74 & & 1.04 & Gaia DR3 \\
7 & 07:40:29.73 & -15:13:03.5 & 12.29 & 0.83 & 55.23 & 11.57 & & 1.24 & Gaia DR3 \\
8 & 07:40:30.48 & -14:34:29.9 & 14.56 & 0.94 & 55.79 & 26.75 & & 1.00 & Gaia DR3 \\
9 & 07:40:38.13 & -14:26:37.3 & 11.81 & 0.86 & 27.76 & 16.80 & & 0.88 & Gaia DR3 \\
10 & 07:40:38.32 & -14:26:23.2 & 14.59 & 0.89 & 87.79 & 10.04 & & 1.01 & Gaia DR3 \\
11 & 07:40:43.08 & -14:53:08.0 & 14.28 & 0.99 & 51.32 & 10.10 & & 1.03 & Gaia DR3 \\
12 & 07:40:44.32 & -15:05:59.4 & 14.58 & 0.95 & 42.62 & 11.19 & & 0.96 & Gaia DR3 \\
13 & 07:40:45.15 & -14:39:57.6 & 11.91 & 0.98 & 62.17 & 20.45 & & 0.96 & Gaia DR3 \\
14 & 07:40:46.38 & -15:17:08.5 & 14.54 & 0.78 & 31.18 & 36.97 & & 0.99 & Gaia DR3 \\
15 & 07:40:47.61 & -14:45:57.3 & 11.14 & 1.00 & 49.09 & 0.50 & & 1.08 & Gaia DR3 \\
16 & 07:40:51.52 & -14:47:26.2 & 14.52 & 0.99 & 47.32 & 13.14 & & 1.01 & Gaia DR3 \\
17 & 07:40:54.69 & -14:22:07.0 & 10.92 & 0.87 & 33.47 & 5.02 & & 0.98 & Gaia DR3 \\
18 & 07:40:58.03 & -14:51:02.6 & 12.02 & 1.00 & 33.56 & 16.43 & & 0.89 & Gaia DR3 \\
19 & 07:40:59.49 & -14:43:59.9 & 13.93 & 0.99 & 39.19 & 11.74 & & 0.99 & Gaia DR3 \\
20 & 07:41:00.64 & -14:22:17.3 & 10.42 & 1.00 & 48.26 & 0.19 & & 1.00 & Gaia DR3 \\
21 & 07:41:02.54 & -14:47:47.4 & 10.77 & 1.00 & 46.94 & 4.18 & & 0.98 & Gaia DR3 \\
22 & 07:41:08.71 & -14:51:29.4 & 14.46 & 0.99 & 45.88 & 7.53 & & 1.08 & Gaia DR3 \\
23 & 07:41:11.13 & -14:39:54.0 & 11.01 & 0.98 & 43.55 & 3.19 & & 1.04 & Gaia DR3 \\
24 & 07:41:11.27 & -14:52:28.1 & 11.64 & 0.99 & 41.83 & 11.29 & & 0.83 & Gaia DR3 \\
25 & 07:41:11.90 & -15:01:39.3 & 11.99 & 0.99 & 37.49 & 12.64 & & 0.93 & Gaia DR3 \\
26 & 07:41:16.18 & -14:56:18.7 & 14.36 & 0.96 & 39.52 & 7.81 & & 1.00 & Gaia DR3 \\
27 & 07:41:16.86 & -14:32:56.8 & 14.23 & 0.95 & 7.07 & 18.20 & & 0.91 & Gaia DR3 \\
28 & 07:41:17.10 & -14:47:30.0 & 11.91 & 0.97 & 60.18 & 17.01 & & 0.86 & Gaia DR3 \\
29 & 07:41:17.35 & -14:51:23.0 & 14.39 & 0.70 & 43.12 & 8.62 & & 1.01 & Gaia DR3 \\
30 & 07:41:17.40 & -14:49:24.7 & 14.54 & 1.00 & 75.44 & 8.85 & & 0.95 & Gaia DR3 \\
31 & 07:41:19.43 & -14:48:47.5 & 9.88 & 1.00 & 53.63 & 4.96 & & 1.10 & Gaia DR3 \\
32 & 07:41:19.96 & -14:54:22.9 & 10.60 & 1.00 & 51.65 & 3.80 & & 1.17 & Gaia DR3 \\
33 & 07:41:21.31 & -14:38:17.5 & 11.04 & 1.00 & 48.33 & 0.29 & & 0.96 & Gaia DR3 \\
34 & 07:41:22.03 & -14:57:42.6 & 14.15 & 0.99 & 38.12 & 9.99 & & 0.94 & Gaia DR3 \\
35 & 07:41:22.90 & -14:49:11.1 & 8.63 & 0.97 & 44.01 & 0.98 & & 1.05 & Gaia DR3 \\
36 & 07:41:23.53 & -14:45:53.8 & 10.26 & 1.00 & 46.82 & 2.04 & & 1.14 & Gaia DR3 \\
37 & 07:41:24.21 & -15:06:29.7 & 14.52 & 0.99 & 57.87 & 10.88 & & 1.01 & Gaia DR3 \\
38 & 07:41:25.93 & -14:41:13.6 & 11.30 & 0.95 & 45.79 & 6.74 & & 1.16 & Gaia DR3 \\
39 & 07:41:26.73 & -14:34:57.1 & 14.48 & 0.98 & 91.19 & 17.63 & & 0.96 & Gaia DR3 \\
40 & 07:41:27.44 & -14:41:13.7 & 14.63 & 1.00 & 21.41 & 12.05 & & 0.96 & Gaia DR3 \\
41 & 07:41:27.84 & -14:51:54.0 & 11.43 & 1.00 & 32.47 & 27.15 & & 0.99 & Gaia DR3 \\
42 & 07:41:28.19 & -14:45:40.1 & 12.02 & 0.96 & 76.11 & 20.16 & & 0.90 & Gaia DR3 \\
43 & 07:41:28.53 & -14:54:17.4 & 10.30 & 0.99 & 42.60 & 2.37 & & 1.25 & Gaia DR3 \\
44 & 07:41:28.97 & -14:47:36.5 & 10.71 & 1.00 & 68.37 & 12.85 & & 0.93 & Gaia DR3 \\
45 & 07:41:29.35 & -14:47:18.8 & 14.53 & 1.00 & 79.20 & 12.54 & & 1.00 & Gaia DR3 \\
46 & 07:41:29.66 & -14:48:59.8 & 11.99 & 0.99 & 53.87 & 22.25 & & 0.91 & Gaia DR3 \\
47 & 07:41:29.97 & -14:47:09.3 & 12.19 & 0.99 & 101.98 & 21.59 & & 1.26 & Gaia DR3 \\
48 & 07:41:30.00 & -14:53:20.4 & 11.24 & 0.99 & 24.26 & 7.26 & & 1.14 & Gaia DR3 \\
49 & 07:41:30.55 & -14:52:59.1 & 14.34 & 1.00 & 50.49 & 8.45 & & 1.23 & Gaia DR3 \\
50 & 07:41:30.55 & -14:53:53.9 & 11.24 & 1.00 & 47.67 & 9.25 & & 1.10 & RAVE \\
51 & 07:41:30.90 & -14:56:22.0 & 11.47 & 0.97 & 45.22 & 6.99 & & 0.78 & Gaia DR3 \\
52 & 07:41:31.39 & -14:20:47.4 & 14.09 & 0.88 & 43.68 & 11.76 & & 1.03 & Gaia DR3 \\
53 & 07:41:31.71 & -15:02:37.1 & 11.51 & 1.00 & 48.44 & 8.65 & & 0.91 & Gaia DR3 \\
54 & 07:41:32.00 & -14:51:48.4 & 10.78 & 0.99 & 54.59 & 4.41 & & 1.08 & Gaia DR3 \\
55 & 07:41:32.05 & -14:57:37.0 & 14.45 & 0.95 & 32.16 & 10.81 & & 0.97 & Gaia DR3 \\
56 & 07:41:32.64 & -14:50:58.4 & 11.76 & 1.00 & 17.88 & 17.66 & & 0.97 & Gaia DR3 \\
57 & 07:41:33.13 & -14:50:12.8 & 11.91 & 1.00 & 21.49 & 17.26 & & 0.83 & Gaia DR3 \\
58 & 07:41:33.16 & -14:40:33.9 & 14.52 & 0.99 & 45.66 & 12.26 & & 1.04 & Gaia DR3 \\
59 & 07:41:33.19 & -14:47:41.7 & 11.74 & 1.00 & 26.12 & 16.69 & & 0.98 & Gaia DR3 \\
60 & 07:41:34.67 & -14:51:31.0 & 10.41 & 1.00 & 50.01 & 2.50 & & 1.01 & Gaia DR3 \\
61 & 07:41:35.23 & -14:45:49.0 & 11.01 & 1.00 & 43.11 & 7.06 & & 0.94 & Gaia DR3 \\
62 & 07:41:35.66 & -15:05:09.8 & 14.55 & 0.80 & 43.80 & 17.80 & & 0.97 & Gaia DR3 \\
63 & 07:41:35.67 & -14:54:27.0 & 14.45 & 0.99 & 4.82 & 19.67 & & 1.03 & Gaia DR3 \\
64 & 07:41:36.88 & -15:22:19.6 & 13.78 & 0.73 & 23.95 & 4.61 & & 1.07 & Gaia DR3 \\
65 & 07:41:36.90 & -14:26:11.2 & 10.28 & 1.00 & 49.64 & 0.18 & & 0.97 & Gaia DR3 \\
66 & 07:41:37.26 & -14:49:31.1 & 12.04 & 0.99 & 41.39 & 22.98 & & 1.00 & Gaia DR3 \\
67 & 07:41:37.83 & -14:48:20.2 & 12.01 & 1.00 & 23.76 & 33.30 & & 0.97 & Gaia DR3 \\
68 & 07:41:38.71 & -14:49:07.9 & 11.74 & 1.00 & 39.56 & 12.44 & & 1.09 & Gaia DR3 \\
69 & 07:41:38.97 & -14:40:55.7 & 11.54 & 1.00 & 41.44 & 7.34 & & 1.08 & RAVE \\
70 & 07:41:40.01 & -14:44:13.9 & 11.88 & 0.99 & 37.81 & 11.97 & & 1.26 & Gaia DR3 \\
71 & 07:41:40.07 & -14:59:34.3 & 14.58 & 1.00 & 40.92 & 25.68 & & 0.95 & Gaia DR3 \\
72 & 07:41:40.18 & -14:59:26.7 & 14.42 & 0.98 & 9.50 & 15.58 & & 1.09 & Gaia DR3 \\
73 & 07:41:40.70 & -14:48:02.0 & 11.39 & 1.00 & 48.80 & 11.74 & & 1.02 & Gaia DR3 \\
74 & 07:41:41.31 & -14:39:53.2 & 11.33 & 1.00 & 45.71 & 8.09 & & 0.96 & Gaia DR3 \\
75 & 07:41:41.41 & -14:47:48.5 & 11.65 & 1.00 & 77.44 & 19.50 & & 0.88 & Gaia DR3 \\
76 & 07:41:41.95 & -14:47:15.8 & 11.29 & 0.99 & 45.42 & 10.89 & & 1.08 & Gaia DR3 \\
77 & 07:41:42.12 & -14:53:32.0 & 14.59 & 0.97 & 78.68 & 19.28 & & 0.97 & Gaia DR3 \\
78 & 07:41:42.14 & -14:45:44.3 & 14.39 & 0.99 & 33.69 & 25.18 & & 1.03 & Gaia DR3 \\
79 & 07:41:42.86 & -14:57:02.3 & 11.08 & 0.99 & 35.76 & 5.12 & & 0.87 & Gaia DR3 \\
80 & 07:41:43.60 & -14:58:29.5 & 11.13 & 1.00 & 52.39 & 3.97 & & 0.93 & Gaia DR3 \\
81 & 07:41:43.96 & -15:00:21.1 & 14.56 & 1.00 & 33.75 & 11.54 & & 0.86 & Gaia DR3 \\
82 & 07:41:44.53 & -15:16:00.8 & 14.17 & 0.91 & 52.74 & 11.72 & & 0.93 & Gaia DR3 \\
83 & 07:41:44.92 & -14:58:35.0 & 14.54 & 0.99 & 42.82 & 8.56 & & 1.01 & Gaia DR3 \\
84 & 07:41:45.12 & -14:50:02.0 & 11.18 & 0.99 & 47.85 & 14.57 & & 1.06 & Gaia DR3 \\
85 & 07:41:45.14 & -14:50:00.0 & 11.84 & 1.00 & -1.41 & 25.07 & & 1.04 & Gaia DR3 \\
86 & 07:41:45.28 & -15:05:26.3 & 14.49 & 0.97 & 26.30 & 11.87 & & 1.07 & Gaia DR3 \\
87 & 07:41:45.73 & -14:50:36.9 & 13.96 & 1.00 & 15.74 & 6.60 & & 0.92 & Gaia DR3 \\
88 & 07:41:48.51 & -14:53:55.9 & 11.93 & 0.99 & 54.35 & 19.57 & & 1.13 & Gaia DR3 \\
89 & 07:41:48.56 & -14:53:02.0 & 10.63 & 0.99 & 48.20 & 1.86 & & 0.91 & Gaia DR3 \\
90 & 07:41:49.02 & -14:28:30.3 & 11.52 & 1.00 & 46.00 & 9.30 & & 1.25 & Gaia DR3 \\
91 & 07:41:49.14 & -14:46:56.2 & 11.16 & 1.00 & 37.48 & 9.09 & & 1.02 & Gaia DR3 \\
92 & 07:41:49.86 & -14:51:15.1 & 10.54 & 1.00 & 35.14 & 6.74 & & 0.90 & Gaia DR3 \\
93 & 07:41:49.91 & -14:45:19.8 & 12.16 & 1.00 & 32.69 & 18.21 & & 0.97 & Gaia DR3 \\
94 & 07:41:50.15 & -14:32:34.1 & 10.94 & 0.98 & 58.39 & 6.56 & & 1.03 & Gaia DR3 \\
95 & 07:41:50.63 & -14:40:07.8 & 11.85 & 0.99 & 43.54 & 13.14 & & 0.89 & Gaia DR3 \\
96 & 07:41:51.53 & -14:54:29.2 & 10.30 & 1.00 & 46.50 & 0.28 & & 0.92 & Gaia DR3 \\
97 & 07:41:51.53 & -14:49:00.1 & 11.57 & 1.00 & 46.29 & 22.48 & & 0.95 & Gaia DR3 \\
98 & 07:41:51.65 & -14:47:11.0 & 11.54 & 1.00 & 52.42 & 17.84 & & 1.03 & Gaia DR3 \\
99 & 07:41:51.93 & -14:46:49.5 & 10.90 & 1.00 & 48.81 & 9.78 & & 1.05 & Gaia DR3 \\
100 & 07:41:52.48 & -15:10:41.2 & 14.40 & 0.94 & 17.58 & 10.50 & & 1.01 & Gaia DR3 \\
101 & 07:41:52.56 & -15:04:30.7 & 14.62 & 0.99 & 22.28 & 11.14 & & 1.03 & Gaia DR3 \\
102 & 07:41:52.56 & -14:52:14.1 & 11.51 & 1.00 & 46.44 & 32.26 & & 1.11 & Gaia DR3 \\
103 & 07:41:52.77 & -14:47:46.1 & 12.13 & 1.00 & 51.81 & 22.93 & & 0.94 & Gaia DR3 \\
104 & 07:41:52.91 & -14:44:32.3 & 11.28 & 1.00 & 40.54 & 10.63 & & 0.99 & Gaia DR3 \\
105 & 07:41:53.43 & -14:45:43.0 & 14.22 & 1.00 & 41.13 & 7.39 & & 1.05 & Gaia DR3 \\
106 & 07:41:54.27 & -14:57:20.6 & 11.94 & 1.00 & 37.88 & 15.30 & & 0.92 & Gaia DR3 \\
107 & 07:41:54.49 & -14:50:11.6 & 11.25 & 1.00 & 45.31 & 11.53 & & 1.33 & Gaia DR3 \\
108 & 07:41:54.50 & -15:05:15.2 & 11.65 & 1.00 & 47.07 & 8.43 & & 0.93 & RAVE \\
109 & 07:41:55.76 & -14:56:34.8 & 11.82 & 1.00 & 31.15 & 13.66 & & 0.82 & Gaia DR3 \\
110 & 07:41:57.04 & -14:25:44.8 & 14.30 & 0.92 & 107.20 & 14.63 & & 0.96 & Gaia DR3 \\
111 & 07:41:57.32 & -14:30:28.4 & 14.42 & 0.97 & 49.87 & 18.80 & & 0.97 & Gaia DR3 \\
112 & 07:41:58.01 & -14:59:26.0 & 12.02 & 1.00 & 54.16 & 16.62 & & 0.84 & Gaia DR3 \\
113 & 07:41:58.39 & -14:45:27.6 & 14.45 & 0.93 & 88.70 & 10.57 & & 0.97 & Gaia DR3 \\
114 & 07:41:58.43 & -14:49:24.8 & 10.25 & 0.99 & 57.35 & 2.68 & & 0.92 & Gaia DR3 \\
115 & 07:42:00.54 & -14:27:27.7 & 14.55 & 0.94 & 53.98 & 23.28 & & 0.98 & Gaia DR3 \\
116 & 07:42:02.55 & -14:46:26.8 & 11.77 & 0.99 & 40.33 & 10.51 & & 0.99 & Gaia DR3 \\
117 & 07:42:02.98 & -14:45:03.0 & 11.31 & 0.98 & 49.98 & 6.82 & & 0.94 & Gaia DR3 \\
118 & 07:42:03.02 & -14:43:43.3 & 12.10 & 1.00 & 44.69 & 9.38 & & 0.92 & Gaia DR3 \\
119 & 07:42:03.12 & -14:53:02.7 & 10.29 & 1.00 & 44.62 & 2.51 & & 0.96 & Gaia DR3 \\
120 & 07:42:03.51 & -14:55:41.7 & 11.73 & 0.85 & 55.39 & 26.82 & & 0.86 & Gaia DR3 \\
121 & 07:42:03.55 & -14:50:39.4 & 14.44 & 1.00 & 59.03 & 17.08 & & 1.00 & Gaia DR3 \\
122 & 07:42:04.35 & -14:57:08.2 & 11.43 & 1.00 & 41.47 & 10.31 & & 0.85 & RAVE \\
123 & 07:42:05.75 & -15:07:16.2 & 14.52 & 0.99 & 57.36 & 12.98 & & 1.01 & Gaia DR3 \\
124 & 07:42:05.93 & -14:44:33.6 & 10.54 & 1.00 & 49.82 & 1.20 & & 0.96 & Gaia DR3 \\
125 & 07:42:08.78 & -14:36:59.2 & 13.93 & 0.98 & 65.51 & 7.65 & & 0.98 & Gaia DR3 \\
126 & 07:42:08.90 & -14:51:04.0 & 11.74 & 1.00 & 39.50 & 19.23 & & 0.88 & RAVE \\
127 & 07:42:10.14 & -14:38:51.2 & 10.91 & 0.99 & 49.41 & 5.55 & & 1.18 & Gaia DR3 \\
128 & 07:42:10.31 & -14:47:13.1 & 11.02 & 0.99 & 41.06 & 3.35 & & 1.08 & Gaia DR3 \\
129 & 07:42:10.68 & -14:41:12.0 & 14.54 & 0.99 & 54.92 & 10.16 & & 0.98 & Gaia DR3 \\
130 & 07:42:10.73 & -14:30:59.3 & 11.09 & 1.00 & 38.44 & 6.35 & & 1.01 & Gaia DR3 \\
131 & 07:42:11.40 & -14:46:42.0 & 14.08 & 0.99 & 33.88 & 22.88 & & 1.10 & Gaia DR3 \\
132 & 07:42:11.92 & -14:48:06.2 & 14.05 & 0.98 & -38.86 & 33.83 & & 1.38 & Gaia DR3 \\
133 & 07:42:12.25 & -14:44:20.2 & 11.84 & 1.00 & 52.15 & 20.97 & & 0.98 & Gaia DR3 \\
134 & 07:42:12.90 & -14:55:18.0 & 11.85 & 1.00 & 54.23 & 11.76 & & 0.82 & Gaia DR3 \\
135 & 07:42:13.91 & -14:44:40.4 & 14.32 & 0.99 & 52.38 & 19.75 & & 1.25 & Gaia DR3 \\
136 & 07:42:16.15 & -14:49:44.4 & 10.58 & 1.00 & 47.42 & 1.21 & & 1.04 & Gaia DR3 \\
137 & 07:42:16.74 & -14:28:27.9 & 14.38 & 0.92 & 59.86 & 10.11 & & 1.06 & Gaia DR3 \\
138 & 07:42:17.59 & -14:56:09.8 & 10.93 & 1.00 & 46.66 & 6.27 & & 1.01 & RAVE \\
139 & 07:42:20.34 & -14:58:59.0 & 13.49 & 0.98 & 45.57 & 10.48 & & 1.05 & Gaia DR3 \\
140 & 07:42:21.54 & -14:27:24.5 & 14.29 & 0.79 & 63.53 & 13.18 & & 1.01 & Gaia DR3 \\
141 & 07:42:22.57 & -14:50:53.9 & 14.30 & 0.99 & 68.24 & 14.05 & & 1.06 & Gaia DR3 \\
142 & 07:42:23.88 & -15:17:44.3 & 10.84 & 1.00 & 48.69 & 0.21 & & 1.03 & Gaia DR3 \\
143 & 07:42:25.46 & -14:14:56.0 & 13.97 & 0.69 & 47.63 & 9.18 & & 0.94 & Gaia DR3 \\
144 & 07:42:25.68 & -15:20:05.6 & 11.47 & 0.88 & 51.17 & 11.62 & & 0.79 & Gaia DR3 \\
145 & 07:42:26.22 & -14:51:30.4 & 11.19 & 1.00 & 34.83 & 5.87 & & 1.06 & RAVE \\
146 & 07:42:26.39 & -14:26:20.2 & 10.94 & 0.90 & 56.10 & 9.15 & & 1.04 & Gaia DR3 \\
147 & 07:42:26.59 & -14:51:02.4 & 14.38 & 1.00 & 48.36 & 14.70 & & 1.05 & Gaia DR3 \\
148 & 07:42:30.32 & -14:57:12.2 & 12.19 & 0.99 & 35.84 & 27.67 & & 1.09 & Gaia DR3 \\
149 & 07:42:31.50 & -14:36:53.1 & 13.71 & 0.97 & 52.71 & 10.94 & & 0.94 & Gaia DR3 \\
150 & 07:42:31.53 & -14:45:47.0 & 14.32 & 0.99 & 45.62 & 10.30 & & 1.00 & Gaia DR3 \\
151 & 07:42:33.95 & -15:03:32.7 & 14.43 & 0.95 & 17.58 & 9.35 & & 0.99 & Gaia DR3 \\
152 & 07:42:34.06 & -14:49:42.9 & 14.15 & 0.99 & -49.55 & 15.61 & & 0.94 & Gaia DR3 \\
153 & 07:42:35.36 & -15:02:48.6 & 11.65 & 1.00 & 45.26 & 10.70 & & 1.01 & Gaia DR3 \\
154 & 07:42:41.24 & -14:59:51.4 & 10.95 & 1.00 & 48.65 & 0.29 & & 0.99 & Gaia DR3 \\
155 & 07:42:41.67 & -15:18:23.3 & 11.03 & 0.86 & 47.90 & 3.10 & & 0.89 & Gaia DR3 \\
156 & 07:42:44.98 & -14:39:10.5 & 14.38 & 0.96 & 54.83 & 8.97 & & 1.04 & Gaia DR3 \\
157 & 07:42:48.31 & -15:02:11.6 & 14.30 & 0.97 & 63.27 & 8.68 & & 0.97 & Gaia DR3 \\
158 & 07:42:51.31 & -14:49:14.8 & 14.49 & 0.99 & 34.66 & 8.86 & & 0.95 & Gaia DR3 \\
159 & 07:42:51.81 & -14:44:11.7 & 10.67 & 1.00 & 34.51 & 4.08 & & 1.18 & RAVE \\
160 & 07:42:56.74 & -14:39:40.9 & 13.93 & 0.92 & 57.56 & 12.90 & & 0.98 & Gaia DR3 \\
161 & 07:42:58.08 & -15:10:13.7 & 11.20 & 0.89 & 44.47 & 5.22 & & 1.28 & Gaia DR3 \\
162 & 07:42:58.97 & -14:54:53.1 & 14.50 & 0.82 & 40.87 & 15.52 & & 1.03 & Gaia DR3 \\
163 & 07:42:59.19 & -14:52:55.6 & 11.88 & 0.97 & 48.76 & 13.06 & & 0.94 & Gaia DR3 \\
164 & 07:43:04.47 & -14:59:50.1 & 14.39 & 0.95 & 64.06 & 10.13 & & 0.97 & Gaia DR3 \\
165 & 07:43:13.79 & -14:29:59.9 & 10.64 & 0.64 & 39.15 & 3.92 & & 1.17 & Gaia DR3 \\
166 & 07:43:15.04 & -14:58:32.1 & 11.49 & 0.91 & 68.72 & 15.05 & & 1.03 & Gaia DR3 \\
167 & 07:43:16.11 & -14:36:46.8 & 14.33 & 0.88 & 55.20 & 15.14 & & 1.00 & Gaia DR3 \\
168 & 07:43:16.14 & -14:52:30.2 & 11.48 & 0.66 & 43.12 & 9.95 & & 1.40 & Gaia DR3 \\
169 & 07:43:26.11 & -15:01:25.8 & 14.33 & 0.86 & 39.70 & 11.14 & & 1.02 & Gaia DR3 \\
170 & 07:43:37.56 & -14:55:50.8 & 11.77 & 0.84 & 42.55 & 32.81 & & 0.96 & Gaia DR3 \\
171 & 07:43:38.97 & -14:49:20.5 & 12.06 & 0.84 & 40.80 & 22.38 & & 0.93 & Gaia DR3 \\
172 & 07:43:40.61 & -14:30:49.5 & 13.34 & 0.70 & 1.70 & 2.82 & & 0.97 & Gaia DR3 \\
173 & 07:43:49.53 & -15:14:24.1 & 13.88 & 0.64 & 42.68 & 9.27 & & 0.97 & Gaia DR3 \\
174 & 07:43:50.00 & -15:05:06.5 & 14.38 & 0.76 & 9.27 & 9.93 & & 1.03 & Gaia DR3 \\
175 & 07:43:56.02 & -15:07:14.3 & 9.35 & 0.62 & 49.16 & 0.37 & & 0.93 & Gaia DR3 \\
\hline
\end{tabular}
\label{tab:NGC_2437}
\end{table*}



